Submodular Cost Submodular Cover with an Approximate Oracle

In this work, we study the Submodular Cost Submodular Cover problem, which is to minimize the submodular cost required to ensure that the submodular benefit function exceeds a given threshold. Existing approximation ratios for the greedy algorithm assume a value oracle to the benefit function. However, access to a value oracle is not a realistic assumption for many applications of this problem, where the benefit function is difficult to compute. We present two incomparable approximation ratios for this problem with an approximate value oracle and demonstrate that the ratios take on empirically relevant values through a case study with the Influence Threshold problem in online social networks.

==> Sections/conclusions.tex <==

\section{Conclusions and Future Work}
%\subsubsection{Tightness of the Ratios of Theorem \ref{ratio} and Theorem \ref{ratio2}}
In this work, we have studied SCSC
when access to the benefit function $f$ is restricted to an approximate oracle. 
We have provided two incomparable approximation ratios, the first of which reduces,
up to a small constant factor,
to the current state-of-the-art ratio for SCSC when the oracle error goes to zero.
The second ratio is easier to bound in practice, and we demonstrate this
fact under a range of different levels of oracle error
in the context of the influence threshold application. 

When applied to the classical set cover problem, which is a special case of 
SCSC, our ratios are nearly tight. For fixed oracle error $\epsilon$ and
arbitrary submodular cost, the tightness of the ratios of Theorem \ref{ratio} and
\ref{ratio2} is an open problem. Furthermore, in this work, we have considered
adversarial oracle error; that is, no additional assumptions on the oracle error have
been made. As a result, the oracle error needs to be relatively small for our bounds
to be meaningful. 
Under more strict assumptions, {i.e.} that the oracle
error follows some probability distribution, it is likely that approximation ratios
under larger oracle error could be developed for SCSC. 
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main.tex"
%%% End:


